A Survey on Quantum Reinforcement Learning

Quantum reinforcement learning is an emerging field at the intersection of quantum computing and machine learning. While we intend to provide a broad overview of the literature on quantum reinforcement learning - our interpretation of this term will be clarified below - we put particular emphasis on recent developments. With a focus on already available noisy intermediate-scale quantum devices, these include variational quantum circuits acting as function approximators in an otherwise classical reinforcement learning setting. In addition, we survey quantum reinforcement learning algorithms based on future fault-tolerant hardware, some of which come with a provable quantum advantage. We provide both a birds-eye-view of the field, as well as summaries and reviews for selected parts of the literature.

==> Tables/Chen_2022a.tex <==
 \begin{table}[ht]
    \centering
    \begin{minipage}{\textwidth}
        \renewcommand\footnoterule{}
        \renewcommand{\thefootnote}{\alph{footnote}}
    \caption*{\textbf{Algorithmic Characteristics - Chen et al.}~\cite{Chen_2022a}}
    \small
    \begin{tabular*}{\textwidth}{p{\dimexpr 0.19\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.14\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.15\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.22\textwidth-2\tabcolsep}}
        \toprule
        \centering\multirow{2}{*}{\textbf{Environment}} & \centering\textbf{Algorithm} & \centering\textbf{Quantum} & \centering\textbf{State} & \centering\textbf{Action} & \centering\multirow{2}{*}{\textbf{Qubits}} & \centering\textbf{Parameterized} \tabularnewline
        & \centering\textbf{Type} & \centering\textbf{Component} & \centering\textbf{Space} & \centering\textbf{Space} & & \centering\textbf{~Gates}\footnotemark[1] \tabularnewline
        \midrule
        \midrule
        %%%% ROW 1
        \centering\texttt{CartPole} &
        \centering\multirow{2}{*}{\gls{dql}\footnotemark[1]} &
        \centering\multirow{2}{*}{$Q$-function} &
        \centering\tiny{continuous} &
        \centering\tiny{discrete} &
        \centering\multirow{2}{*}{$2$} &
        \centering $3$ (encoding) \tabularnewline
        \centering (OpenAI Gym) &
        &
        &
        \centering $4$-dim &
        \centering $2$ &
        &
        \centering $26$ (weights) \tabularnewline
        \midrule
        %%%%% ROW2
        \centering\texttt{MiniGrid} &
        \centering\multirow{2}{*}{\gls{dql}\footnotemark[1]} &
        \centering\multirow{2}{*}{$Q$-function} &
        \centering\tiny{discrete} &
        \centering\tiny{discrete} &
        \centering\multirow{2}{*}{$8$} &
        \centering $8$ (encoding)\footnotemark[2] \tabularnewline
        \centering (OpenAI Gym) &
        &
        &
        \centering $147$ &
        \centering $6$ &
        &
        \centering $24$ (weights) \tabularnewline
        \bottomrule
    \end{tabular*}
    \footnotetext[1]{~the standard \gls{qrl} pipeline is reformulated to allow training via evolutionary optimization;}
    \footnotetext[2]{~this does not include parameters of the \gls{tn} for dimensionality reduction; details are not stated;}
    \end{minipage}
\end{table}

==> Tables/Hsiao_2022.tex <==
 \begin{table}[h!]
    \centering
    \begin{minipage}{\textwidth}
        \renewcommand\footnoterule{}
        \renewcommand{\thefootnote}{\alph{footnote}}
    \caption*{\textbf{Algorithmic Characteristics - Hsiao et al.}~\cite{Hsiao_2022}}
    \small
    \begin{tabular*}{\textwidth}{p{\dimexpr 0.19\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.14\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.15\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.22\textwidth-2\tabcolsep}}
        \toprule
        \centering\multirow{2}{*}{\textbf{Environment}} & \centering\textbf{Algorithm} & \centering\textbf{Quantum} & \centering\textbf{State} & \centering\textbf{Action} & \centering\multirow{2}{*}{\textbf{Qubits}} & \centering\textbf{Parameterized} \tabularnewline
        & \centering\textbf{Type} & \centering\textbf{Component} & \centering\textbf{Space} & \centering\textbf{Space} & & \centering\textbf{~Gates}\footnotemark[1] \tabularnewline
        \midrule
        \midrule
        %%%% ROW 1
        \centering\texttt{CartPole} &
        \centering\multirow{2}{*}{\gls{ppo}} &
        \centering\multirow{2}{*}{Policy} &
        \centering\tiny{continuous} &
        \centering\tiny{discrete} &
        \centering\multirow{2}{*}{$4$} &
        \centering\multirow{2}{*}{$12$} \tabularnewline
        \centering (OpenAI Gym) &
        &
        &
        \centering $4$-dim &
        \centering $2$ &
        &
        \tabularnewline
        \midrule
        %%%%% ROW 2
        \centering\texttt{Acrobot} &
        \centering\multirow{2}{*}{\gls{ppo}} &
        \centering\multirow{2}{*}{Policy} &
        \centering\tiny{continuous} &
        \centering\tiny{discrete} &
        \centering\multirow{2}{*}{$6$} &
        \centering\multirow{2}{*}{$18$} \tabularnewline
        \centering (OpenAI Gym) &
        &
        &
        \centering $6$-dim &
        \centering $3$ &
        &
        \tabularnewline
        \midrule
        %%%%% ROW 3
        \centering\texttt{LunarLander} &
        \centering\multirow{2}{*}{\gls{ppo}} &
        \centering\multirow{2}{*}{Policy} &
        \centering\tiny{continuous} &
        \centering\tiny{discrete} &
        \centering\multirow{2}{*}{$8$} &
        \centering\multirow{2}{*}{$72$} \tabularnewline
        \centering (OpenAI Gym) &
        &
        &
        \centering $8$-dim &
        \centering $4$ &
        &
        \tabularnewline
        \bottomrule
    \end{tabular*}
    \footnotetext[1]{~this entails encoding and variational parameters; an appended \gls{nn} adds classical parameters;}
    \end{minipage}
\end{table}

==> Tables/Kimura_2021.tex <==
 \begin{table}[ht]
    \centering
    \begin{minipage}{\textwidth}
        \renewcommand\footnoterule{}
        \renewcommand{\thefootnote}{\alph{footnote}}
    \caption*{\textbf{Algorithmic Characteristics - Kimura et al.}~\cite{Kimura_2021}}
    \small
    \begin{tabular*}{\textwidth}{p{\dimexpr 0.19\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.14\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.15\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.22\textwidth-2\tabcolsep}}
        \toprule
        \centering\multirow{2}{*}{\textbf{Environment}} & \centering\textbf{Algorithm} & \centering\textbf{Quantum} & \centering\textbf{State} & \centering\textbf{Action} & \centering\multirow{2}{*}{\textbf{Qubits}} & \centering\textbf{Parameterized} \tabularnewline
        & \centering\textbf{Type} & \centering\textbf{Component} & \centering\textbf{Space} & \centering\textbf{Space} & & \centering\textbf{~Gates}\footnotemark[1] \tabularnewline
        \midrule
        \midrule
        %%%% ROW 1
        \centering\multirow{3}{*}{\begin{tabular}{@{}c@{}}\texttt{PO Maze}\\(see \cite{Kimura_2021})\end{tabular}} &
        \centering complex- &
        \centering\multirow{3}{*}{$\overset{.}{Q}$-function} &
        \centering\multirow{3}{*}{\begin{tabular}{@{}c@{}}{\tiny{discrete}}\\$18$\end{tabular}} &
        \centering\multirow{3}{*}{\begin{tabular}{@{}c@{}}{\tiny{discrete}}\\$4$\end{tabular}} &
        \centering\multirow{3}{*}{$6$} &
        \centering $6 \times 2$ (encoding) \tabularnewline
         &
        \centering valued &
        &
        &
        &
        &
        \centering $6 \times 4 \times 2$ (weights) \tabularnewline
        &
        \centering \gls{dql} &
        &
        &
        &
        &
        \centering $6 \times 3$ (decoding) \tabularnewline
        \bottomrule
    \end{tabular*}
    \footnotetext[1]{~encoding and decoding gates: $qubits \times per\_qubit$; variational gates: $qubits \times layers \times per\_qubit\_per\_layer$;}
    \end{minipage}
\end{table}

==> Tables/Sanches_2022.tex <==
 \begin{table}[ht]
    \centering
    \begin{minipage}{\textwidth}
        \renewcommand\footnoterule{}
        \renewcommand{\thefootnote}{\alph{footnote}}
    \caption*{\textbf{Algorithmic Characteristics - Sanches et al.}~\cite{Sanches_2022}}
    \small
    \begin{tabular*}{\textwidth}{p{\dimexpr 0.19\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.14\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.15\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.1\textwidth-2\tabcolsep-\arrayrulewidth}|p{\dimexpr 0.22\textwidth-2\tabcolsep}}
        \toprule
        \centering\multirow{2}{*}{\textbf{Environment}} & \centering\textbf{Algorithm} & \centering\textbf{Quantum} & \centering\textbf{State} & \centering\textbf{Action} & \centering\multirow{2}{*}{\textbf{Qubits}} & \centering\textbf{Parameterized} \tabularnewline
        & \centering\textbf{Type} & \centering\textbf{Component} & \centering\textbf{Space} & \centering\textbf{Space} & & \centering\textbf{Gates} \tabularnewline
        \midrule
        \midrule
        %%%% ROW 1
        \centering\multirow{2}{*}{\texttt{\gls{vrp}}\footnotemark[1]} &
        \centering\multirow{2}{*}{\scriptsize{REINFORCE}} &
        \centering Attention- &
        \centering\tiny{continuous} &
        \centering\multirow{2}{*}{$--$} &
        \centering\multirow{2}{*}{$4$} &
        \centering $4$ (encoding) \tabularnewline
        &
        &
        \centering Head &
        \centering $2$-dim &
        &
        &
        \centering $2$ (weights) \tabularnewline
        \bottomrule
    \end{tabular*}
    \footnotetext[1]{~several instances of this component are used as subroutine of a complex classical model;}
    \end{minipage}
\end{table}
